On the Impact of Hardware Impairments on RIS-aided Localization

We investigate a reconfigurable intelligent surface (RIS)-aided near-field localization system with single-antenna user equipment (UE) and base station (BS) under hardware impairments by considering a practical phase-dependent RIS amplitude variations model. To analyze the localization performance under the mismatch between the practical model and the ideal model with unit-amplitude RIS elements, we employ the misspecified Cram\'{e}r-Rao bound (MCRB). Based on the MCRB derivation, the lower bound (LB) on the mean-squared error for estimation of UE position is evaluated and shown to converge to the MCRB at low signal-to-noise ratios (SNRs). Simulation results indicate more severe performance degradation due to the model misspecification with increasing SNR. In addition, the mismatched maximum likelihood (MML) estimator is derived and found to be tight to the LB in the high SNR regime. Finally, we observe that the model mismatch can lead to an order-of-magnitude localization performance loss at high SNRs.

==> listofitems.tex <==
% !TeX encoding = ISO-8859-1
% Ce fichier contient le code de l'extension "listofitems"
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                                                    %
\def\loiname                 {listofitems}                           %
\def\loiver                      {1.63}                              %
%                                                                    %
\def\loidate                  {2019/08/21}                           %
%                                                                    %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                                                    %
% Author     : Christian Tellechea, Steven B. Segletes (contributor) %
% Status     : Maintained                                            %
% Maintainer : Christian Tellechea                                   %
% Email      : unbonpetit@netc.fr                                    %
%              steven.b.segletes.civ@mail.mil                        %
% Package URL: https://www.ctan.org/pkg/listofitems                  %
% Bug tracker: https://framagit.org/unbonpetit/listofitems/issues    %
% Repository : https://framagit.org/unbonpetit/listofitems/tree/master
% Copyright  : Christian Tellechea 2016-2019                         %
% Licence    : Released under the LaTeX Project Public License v1.3c %
%              or later, see http://www.latex-project.org/lppl.txt   %
% Files      : 1) listofitems.tex                                    %
%              2) listofitems.sty                                    %
%              3) listofitems-fr.tex                                 %
%              4) listofitems-fr.pdf                                 %
%              5) listofitems-en.tex                                 %
%              6) listofitems-en.pdf                                 %
%              7) README                                             %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\expandafter\edef\csname loi_restorecatcode\endcsname{\catcode\number`\_=\number\catcode`\_\relax}
\catcode`\_11

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%% gestion des erreurs + annonce package %%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\unless\ifdefined\loi_fromsty
	\immediate\write -1 {Package: \loidate\space v\loiver\space Grab items in lists using user-specified sep char (CT)}%
\fi

\ifdefined\PackageError
	\def\loi_error#1{\PackageError\loiname{#1}{Read the \loiname\space manual}}% pour LaTeX
\else
	\def\loi_error#1{\errmessage{Package \loiname\space Error: #1^^J}}% pour TeX
\fi

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%% vérification des prérequis %%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\loi_checkprimitive#1#2#3{% Vérifie que #1 est une primitive et sinon, émet le message #2 et exécute #3
	\begingroup
		\edef\__tempa{\meaning#1}\edef\__tempb{\string#1}\expandafter
	\endgroup
	\ifx\__tempa\__tempb\else
		\loi_error{#2}%
		\def\loi_temp{#3}%
		\loi_restorecatcode\expandafter\loi_temp
	\fi
}
\loi_checkprimitive\eTeXversion
	{You are not using an eTeX engine, listofitems cannot work.}
	{\endinput}%
\loi_checkprimitive\expanded
	{the \string\expanded\space primitive is not provided by your TeX engine, listofitems v\loiver\space cannot work: loading listofitems v1.61}
	{\input listofitemsold.tex\relax\endinput}%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%% macros auxiliaires %%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\loi_quark{\loi_quark}
\long\def\loi_identity#1{#1}
\long\def\loi_gobarg#1{}
\long\def\loi_first#1#2{#1}
\long\def\loi_second#1#2{#2}
\long\def\loi_firsttonil#1#2\_nil{#1}
\long\def\loi_antefi#1#2\fi{#2\fi#1}
\long\def\loi_exparg#1#2{\expandafter\loi_exparg_a\expandafter{#2}{#1}}% \loi_exparg{<a>}{<b>} devient <a>{<*b>}
\long\def\loi_exparg_a#1#2{#2{#1}}
\long\def\loi_expafter#1#2{\expandafter\loi_expafter_a\expandafter{#2}{#1}}% \loi_expafter{<a>}{<b>} devient <a><*b>
\long\def\loi_expafter_a#1#2{#2#1}
\def\loi_macroname{\loi_ifinrange\escapechar[[0:255]]{\expandafter\loi_gobarg}{}\string}
\def\loi_argcsname#1#{\loi_argcsname_a{#1}}
\def\loi_argcsname_a#1#2{\loi_expafter{#1}{\csname#2\endcsname}}
\long\def\loi_addtomacro#1#2{\loi_exparg{\def#1}{#1#2}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%% macros de test %%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\long\def\loi_ifnum#1{\ifnum#1\expandafter\loi_first\else\expandafter\loi_second\fi}
\long\def\loi_ifx#1{\ifx#1\expandafter\loi_first\else\expandafter\loi_second\fi}
\long\def\loi_ifempty#1{\loi_exparg\loi_ifx{\expandafter\relax\detokenize{#1}\relax}}
\def\loi_ifstar#1#2{\def\loi_ifstar_a{\loi_ifx{*\loi_nxttok}{\loi_first{#1}}{#2}}\futurelet\loi_nxttok\loi_ifstar_a}
\edef\loi_escapechar{\expandafter\loi_gobarg\string\\}
\long\def\loi_ifcsexpandable#1{% #1 est-il constitué d'une seule sc _développable_ ?
	\loi_ifempty{#1}
		{\loi_second
		}
		{\loi_ifspacefirst{#1}
			{\loi_second% si espace en 1er, faux
			}
			{\csname loi_\if\loi_escapechar\expandafter\loi_firsttonil\detokenize{#1}\_nil first\else second\fi\endcsname
				{\loi_exparg\loi_ifempty{\loi_gobarg#1}% 1 seul arg commençant par "\" ?
					{\def\loi_tempa{#1}\loi_exparg{\def\loi_tempb}{#1}% est-il développable ?
					\expandafter\unless\loi_ifx{\loi_tempa\loi_tempb}%
					}
					{\loi_second
					}%
				}
				{\loi_second
				}%
			}%
		}%
}
\def\loi_ifinrange#1[[#2:#3]]{\expandafter\unless\loi_ifnum{\numexpr(#1-#2)*(#1-#3)>0 }}
\def\loi_ifstring#1#2{% si la chaine #1 est contenue dans #2
	\def\loi_ifstring_a##1#1##2\_nil{\loi_ifempty{##2}\loi_second\loi_first}%
	\loi_ifstring_a#2#1\_nil% appel de la macro auxiliaire
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%% macro \loi_foreach %%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcount\loi_cnt_foreach_nest \loi_cnt_foreach_nest=0
\def\end_foreach{\end_foreach}
\def\loi_def_foreachsep#1{%
	\long\def\loi_foreach##1\in##2##3{%
		\global\advance\loi_cnt_foreach_nest1
		\loi_argcsname\def{loop_code_\number\loi_cnt_foreach_nest}{##3}%
		\loi_foreach_a##1##2#1\end_foreach#1%
		\loi_argcsname\let{loop_code_\number\loi_cnt_foreach_nest}\empty
		\global\advance\loi_cnt_foreach_nest-1
	}%
	\long\def\loi_foreach_a##1##2#1{%
		\def##1{##2}%
		\loi_ifx{\end_foreach##1}
			{}
			{\csname loop_code_\number\loi_cnt_foreach_nest\endcsname% exécute le code
			\loi_foreach_a##1%
			}%
	}%
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%% macros gérant l'appariement %%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\long\def\defpair#1{%
	\let\loi_listofpair\empty
	\loi_ifempty{#1}
		{}
		{\defpair_a{}#1\loi_quark\loi_quark}%
}
\long\def\defpair_a#1#2#3{%
	\loi_ifx{\loi_quark#2}
		{\def\loi_sanitizelist##1,\_nil{\def\loi_listofpair{##1}}%
		\loi_sanitizelist#1\_nil
		}
		{\loi_if_validpair#2#3%
			{\long\def\loi_paired_a{#2}\long\def\loi_paired_b{#3}%
			\loi_ifx{\loi_paired_a\loi_paired_b}
				{\loi_error{Paired tokens must not be equal, the pair \detokenize{#2#3} is ignored}%
				\defpair_a{#1}%
				}
				{\defpair_a{#1#2#3,}%
				}%
			}
			{\loi_error{Invalid paired tokens, the pair "\detokenize{#2}" and "\detokenize{#3}" is ignored}%
			\defpair_a{#1}%
			}%
		}%
}
\long\def\loi_if_validpair#1#2{%
	\def\loi_validpair{1}%
	\loi_if_invalid_pairtoken{#1}{\def\loi_validpair{0}}%
	\loi_if_invalid_pairtoken{#2}{\def\loi_validpair{0}}%
	\loi_ifnum{\loi_validpair=1 }
}
\long\def\loi_if_invalid_pairtoken#1{%
	\loi_ifempty{#1}
		{\loi_identity
		}
		{\loi_ifspacefirst{#1}
			{\loi_identity
			}
			{\loi_exparg\loi_ifempty{\loi_gobarg#1}% 1 seul token ?
				{\ifcat\relax\noexpand#1\expandafter\loi_identity\else\expandafter\loi_gobarg\fi}
				{\loi_identity}% si plusieurs tokens, faux
			}%
		}%
}
\long\def\loi_count_occur#1\in#2:#3{% compte le nombre d'occurrences de #1 dans #2 et met le résultat dans la macro #3
	\long\def\loi_count_occur_a##1##2#1##3\_nil{%
		\loi_ifempty{##3}
			{\def#3{##1}}
			{\expandafter\loi_count_occur_a\number\numexpr##1+1\relax##3\_nil}%
	}%
	\loi_count_occur_a0#2#1\_nil
}
\long\def\loi_check_pair#1#2\in#3{% teste l'appariement de #1 et #2 dans #3
	\loi_ifempty{#3}
		{\loi_second
		}
		{\loi_count_occur#1\in#3:\loi_tempa
		\loi_count_occur#2\in#3:\loi_tempb
		\loi_ifnum{\loi_tempa=\loi_tempb\relax}%
		}%
}
\long\def\loi_grabpaired_expr#1#2#3#4#5{% #1=liste de paires  #2=expression  #3=séparateur   #4=résultat    #5=ce qui reste
	\let#4\empty
	\def\loi_remain{#2#3}%
	\loi_foreach\loi_pair\in{#1}{\expandafter\loi_grabpaired_expr_a\loi_pair{#3}#4}%
	\def\loi_remove_lastsep##1#3\_nil{\def#4{##1}}%
	\expandafter\loi_remove_lastsep#4\_nil
	\loi_expafter{\long\def\loi_grab_remain}#4##1\_nil{%
		\loi_ifempty{##1}
			{\let#5\empty}
			{\loi_exparg{\def#5}{\loi_gobarg##1}}%
	}%
	\loi_grab_remain#2\_nil
}
\long\def\loi_grabpaired_expr_a#1#2#3#4{% #1#2=paire en cours  #3=séparateur   #4=résultat
	\loi_exparg{\loi_check_pair#1#2\in}#4% si les paires sont appariées dans le résultat
		{}% passer à la paire suivante
		{\long\def\loi_grabpaired_expr_b##1#3##2\_nil{%
			\loi_addtomacro#4{##1#3}% ajouter au résultat ce qui est jusqu'au prochain séparateur
			\def\loi_remain{##2}%
			\loi_exparg{\loi_check_pair#1#2\in}{#4}
				{}
				{\loi_ifempty{##2}
					{\loi_error{"\detokenize{#1}" and "\detokenize{#2}" are not paired}}
					{\loi_grabpaired_expr_b##2\_nil}%
				}%
			}%
		\expandafter\loi_grabpaired_expr_b\loi_remain\_nil
		}%
}
\def\insidepair#1#2#3#4{% #1#2=paire  #3=expr  #4=macro reçevant le resultat
	\loi_if_validpair#1#2%
		{\loi_ifcsexpandable{#3}
			{\loi_exparg{\insidepair#1#2}{#3}#4%
			}
			{\loi_check_pair#1#2\in{#3}% si les paires sont appariées dans le résultat
				{\def\insidepair_a##1#1##2\_nil{\insidepair_b##2\_nil{#1}}%
				\def\insidepair_b##1#2##2\_nil##3{%
					\loi_check_pair#1#2\in{##3##1#2}
						{\loi_exparg{\def#4}{\loi_gobarg##3##1}%
						\def\loi_remainafterparen{##2}%
						}%
						{\insidepair_b##2\_nil{##3##1#2}%
						}%
					}%
				\insidepair_a#3\_nil
				}
				{\loi_error{"\detokenize{#1}" and "\detokenize{#2}" are not paired in "#3"}%
				}%
			}%
		}
		{\loi_error{Invalid paired tokens "\detokenize{#1}" and "\detokenize{#2}", empty \string#4 returned}% et bim
		\let#4\empty% voilà, bien fait pour vos gueules
		}%
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%% macro \loi_fornum %%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\loi_fornum#1=#2to#3\do{%
	\edef#1{\number\numexpr#2}%
	\expandafter\loi_fornum_a
		\csname loi_fornum_\string#1\expandafter\endcsname\expandafter
		{\number\numexpr#3\expandafter}%
		\expanded{\ifnum#1<\numexpr#3\relax>+\else<-\fi}%
		#1%
}
\long\def\loi_fornum_a#1#2#3#4#5#6{%
	\def#1{%
		\unless\ifnum#5#3#2\relax
			\loi_antefi{#6\edef#5{\number\numexpr#5#41\relax}#1}%
		\fi}%
	#1%
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%% macro retirant les espaces extrêmes %%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\long\def\loi_ifspacefirst#1{\expandafter\loi_ifspacefirst_a\detokenize{#10} \_nil}
\long\def\loi_ifspacefirst_a#1 #2\_nil{\loi_ifempty{#1}}
\loi_expafter{\def\loi_gobspace}\space{}
\long\def\loi_removefirstspaces#1{\loi_ifspacefirst{#1}{\loi_exparg\loi_removefirstspaces{\loi_gobspace#1}}{\unexpanded{#1}}}%##BUGFIX v1.63
\begingroup
	\catcode0 12
	\long\gdef\loi_removelastspaces#1{\loi_removelastspaces_a#1^^00 ^^00\_nil}
	\long\gdef\loi_removelastspaces_a#1 ^^00{\loi_removelastspaces_b#1^^00}
	\long\gdef\loi_removelastspaces_b#1^^00#2\_nil{\loi_ifspacefirst{#2}{\loi_removelastspaces_a#1^^00 ^^00\_nil}{\unexpanded{#1}}}
\endgroup
\long\def\loi_removeextremespaces#1{\expanded{\loi_exparg\loi_removelastspaces{\expanded{\loi_removefirstspaces{#1}}}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%% macro publique \setsepchar %%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\setsepchar{\futurelet\loi_nxttok\setsepchar_a}
\def\setsepchar_a{\loi_ifx{[\loi_nxttok}\setsepchar_b{\setsepchar_b[/]}}
\long\def\setsepchar_b[#1]#2{% #1=sepcar de <liste des sepcar>  #2=<liste des sepcar>
	\loi_ifempty{#1}
		{\loi_error{Empty separator not allowed, separator "/" used}%
		\setsepchar_b[/]{#2}%
		}
		{\def\loi_currentsep{#1}%
		\_removeextremespacesfalse
		\loi_nestcnt1 % réinitaliser niveau initial à 1
		\def\nestdepth{1}%
		\loi_argcsname\let{loi_previndex[\number\loi_nestcnt]}\empty
		\def\loi_listname{loi_listofsep}%
		\let\loi_def\def \let\loi_edef\edef \let\loi_let\let
		\let\loi_listofpair_saved\loi_list_ofpair
		\let\loi_list_ofpair\empty
		\loi_ifempty{#2}
			{\loi_error{Empty list of separators not allowed, "," used}%
			\readlist_g1{,}%
			}
			{\readlist_g1{#2}%
			}%
		\loi_argcsname\let\nestdepth{loi_listofseplen[0]}%
		\loi_argcsname\let\loi_currentsep{loi_listofsep[1]}% 1er car de séparation
		\let\loi_listofpair\loi_listofpair_saved
		}%
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%% macro normalisant l'index %%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\loi_normalizeindex#1#2{% #1=macroname  #2=liste d'index  --> renvoie {err}{indx norm}
	\loi_ifempty{#2}
		{{}{}}
		{\loi_exparg{\loi_normalizeindex_a1{}}{\number\csname#1nest\endcsname}{#1}#2,\loi_quark,}%
}%
\def\loi_normalizeindex_a#1#2#3#4#5,{% #1=compteur de profondeur #2=index précédents  #3=profondeur max #4=macroname  #5=index courant
	\loi_ifx{\loi_quark#5}
		{\loi_normalizeindex_c#2\loi_quark% supprimer la dernière virgule
		}
		{\loi_ifnum{#1>#3 }
			{\loi_invalidindex{Too deeply nested index, index [.] retained}{#2}% si profondeur trop grande
			}
			{\loi_ifinrange\ifnum\numexpr#5<0 -1*\fi(#5)[[1:\csname #4len[#20]\endcsname]]% si abs(#5) hors de [1,len]
				{\loi_exparg\loi_normalizeindex_b{\number\numexpr#5\ifnum\numexpr#5<0 +\csname #4len[#20]\endcsname+1\fi}{#1}{#2}{#3}{#4}}
				{\loi_invalidindex{#5 is an invalid index, index [.] retained}{#2}}%
			}%
		}%
}
\def\loi_normalizeindex_b#1#2#3{\loi_exparg\loi_normalizeindex_a{\number\numexpr#2+1}{#3#1,}}% #1=index à rajouter  #2=compteur de profondeur #3=index précédents
\def\loi_normalizeindex_c#1,\loi_quark{{}{#1}}
\def\loi_invalidindex#1#2{\loi_ifempty{#2}{\loi_invalidindex_a{#1},}\loi_invalidindex_a{#1}{#2}}
\def\loi_invalidindex_a#1#2{\loi_invalidindex_b#1\loi_quark#2\loi_quark}
\def\loi_invalidindex_b#1[.]#2\loi_quark#3,\loi_quark#4\loi_quark,{{#1[#3]#2}{#3}}% #4= index ignorés

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%% macro publique \readlist %%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcount\loi_nestcnt
\def\greadlist{\let\loi_def\gdef\let\loi_edef\xdef\def\loi_let{\global\let}\readlist_a}%
\def\readlist{\let\loi_def\def\let\loi_edef\edef\let\loi_let\let\readlist_a}
\def\readlist_a{%
	\loi_nestcnt1 % niveau initial = 1
	\loi_argcsname\let{loi_previndex[\number\loi_nestcnt]}\empty
	\loi_ifstar{\_removeextremespacestrue\readlist_b}{\_removeextremespacesfalse\readlist_b}%
}
\long\def\readlist_b#1#2{% #1=macro stockant les éléments  #2=liste des éléments
	\loi_ifcsexpandable{#2}
		{\loi_exparg{\readlist_b#1}{#2}%
		}
		{\loi_edef\loi_listname{\loi_macroname#1}%
		\loi_exparg{\readlist_c#1{#2}}{\loi_listname}%%
		}%
}
\long\def\readlist_c#1#2#3{% #1=macro stockant les éléments  #2=liste des éléments #3=macroname
	\loi_argcsname\loi_let{#3nest}\nestdepth
	\loi_argcsname\loi_def{#3[]}{#2}% la liste entière
	\loi_argcsname\loi_def{#3sep[]}{}% séparateur vide
	\loi_ifempty{#2}
		{\loi_def#1[##1]{}%
		\loi_argcsname\loi_def{#3len}{0}\loi_argcsname\loi_def{#3len[0]}{0}%
		\loi_error{Empty list ignored, nothing to do}%
		}
		{\loi_def#1[##1]{\expanded{\expandafter\readlist_d\expanded{\loi_normalizeindex{#3}{##1}}{#3}}}%
		\loi_argcsname\loi_def{#3sep}[##1]{\expanded{\expandafter\readlist_d\expanded{\loi_normalizeindex{#3}{##1}}{#3sep}}}%
		\readlist_e{#2}%
		\loi_argcsname\loi_argcsname\loi_let{#3len}{#3len[0]}% longueur du niveau 0
		}%
}
\def\readlist_d#1#2#3{%
	\unexpanded\expandafter\expandafter\expandafter{\csname#3[#2]\expandafter\endcsname\expandafter}%
	\expanded{\loi_ifempty{#1}{}{\unexpanded{\unexpanded{\loi_error{#1}}}}}%
}
\def\readlist_e{%
	\loi_argcsname\loi_let\loi_currentsep{loi_listofsep[\number\loi_nestcnt]}%
	\expandafter\readlist_f\loi_currentsep||\_nil
}
\long\def\readlist_f#1||#2\_nil#3{\readlist_g1{#3#1}}% #1=<sep courant simple>  #3=liste -> rajoute un élément vide pour le test \ifempty ci dessous
\long\def\readlist_g#1#2{% #1=compteur d'index  #2=liste d'éléments à examiner terminée par <sep courant simple> >>RIEN laissé après
	\loi_ifempty{#2}
		{\loi_argcsname\loi_edef{\loi_listname len[\csname loi_previndex[\number\loi_nestcnt]\endcsname0]}{\number\numexpr#1-1\relax}%
		\loi_argcsname\loi_let{\loi_listname sep[\csname loi_previndex[\number\loi_nestcnt]\endcsname\number\numexpr#1-1\relax]}\empty% le dernier <sep> est <vide> ##NEW v1.52
		\advance\loi_nestcnt-1
		\loi_argcsname\loi_let\loi_currentsep{loi_listofsep[\number\loi_nestcnt]}%
		}
		{\loi_expafter{\readlist_h{#2}{}}\loi_currentsep||\loi_quark||#2\_nil{#1}% aller isoler le 1er item
		}%
}
\long\def\readlist_h#1#2#3||{% #1=liste restante   #2=<dernier sep utilisé>  #3=<sep courant>
	\loi_ifx{\loi_quark#3}% on a épuisé tous les <séparateurs> ? RESTE à lire <expr+sep1>\_nil{<compteur>}
		{\loi_ifempty{#2}% si #2 vide, aucun <sep utilisé> n'a été trouvé, il reste à lire "<liste complète>\_nil"
			{\long\def\readlist_i##1\_nil##2{\loi_exparg{\readlist_j{##2}{}}{\loi_gobarg##1}{#2}}% ##2=compteur d'index
			}
			{\loi_ifx{\loi_listofpair\empty}% paires définies ?
				{\long\def\readlist_i##1#2##2\_nil##3{\loi_exparg{\readlist_j{##3}{##2}}{\loi_gobarg##1}{#2}}%
				}
				{\long\def\readlist_i##1\_nil##2{%
					\loi_exparg{\loi_exparg\loi_grabpaired_expr\loi_listofpair}{\loi_gobarg##1}{#2}\loi_grabpaired_result\loi_grabpaired_remain
					\loi_exparg{\loi_exparg{\readlist_j{##2}}{\loi_grabpaired_remain}}{\loi_grabpaired_result}{#2}}%{#}
				}%
			}%
		\readlist_i\relax% le \relax meuble l'argument délimité
		}
		{\long\def\readlist_i##1#3##2\_nil{%
			\loi_ifempty{##2}% si <liste restante> ne contient pas le <sep courant>
				{\readlist_h{#1}{#2}% recommencer avec le même <sep utile>
				}%
				{\loi_ifx{\loi_listofpair\empty}% si pas de paires définies
					{\loi_exparg\readlist_h{\loi_gobarg##1#3}{#3}% raccourcir <liste restante> et <sep courant>:=<sep utile>% ##BUGFIX v1.53
					}%
					{\loi_exparg\loi_grabpaired_expr\loi_listofpair{#1#3}{#3}\loi_grabpaired_result\loi_grabpaired_remain
					\loi_ifx{\loi_grabpaired_remain\empty}% si liste non raccourcie #BUGFIX 1.63
						{\loi_exparg\readlist_h{\loi_grabpaired_result}{#2}}% garder le précédent <sep>
						{\loi_exparg\readlist_h{\loi_grabpaired_result}{#3}}%
					}%
				}%
			}%
		\readlist_i\relax#1#3\_nil% ##BUGFIX v1.53
		}%
}
\long\def\readlist_j#1#2#3{% #1=compteur d'index  #2=liste restante  #3=élément courant
	\loi_ifnum{0\loi_exparg\loi_ifspacefirst{\loi_currentsep}{}1\if_removeextremespaces1\fi=11 }% s'il faur retirer les espaces extrêmes
		{\loi_exparg{\loi_exparg{\readlist_k{#1}{#2}}}{\loi_removeextremespaces{#3}}}% redéfinir l'élément courant
		{\readlist_k{#1}{#2}{#3}}%
}
\long\def\readlist_k#1#2#3#4{% #1=compteur d'index  #2=liste restante  #3=élément courant   #4=sep utilisé
	\loi_ifnum{0\if_ignoreemptyitems1\fi\loi_ifempty{#3}1{}=11 }
		{\readlist_g{#1}{#2}% si l'on n'ignore pas les éléments vides
		}%
		{\loi_argcsname\loi_def{\loi_listname[\csname loi_previndex[\number\loi_nestcnt]\endcsname#1]}{#3}% assignation
		\loi_argcsname\loi_def{\loi_listname sep[\csname loi_previndex[\number\loi_nestcnt]\endcsname#1]}{#4}% assignation du <sep> actuel à la macro \<macrolist>sep
		\loi_ifnum{\loi_nestcnt<\nestdepth\relax}% si imbrication max non atteinte
			{\advance\loi_nestcnt1
			\loi_argcsname\edef{loi_previndex[\number\loi_nestcnt]}{\csname loi_previndex[\number\numexpr\loi_nestcnt-1]\endcsname#1,}%
			\readlist_e{#3}% recommencer avec l'élément courant
			}
			{}%
		\loi_exparg\readlist_g{\number\numexpr#1+1}{#2}% puis chercher l'élément suivant dans la liste restante
		}%
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%% macro \listlen %%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\listlen#1[#2]{%
	\expanded{%
		\loi_ifempty{#2}
			{\csname\loi_macroname#1len[0]\endcsname}
			{\loi_exparg\listlen_a{\expanded{\loi_macroname#1}}{#2}}%
	}%
}
\def\listlen_a#1#2{% #1=macro name   #2=index non normalisé    prendre <profondeur max-1>
	\expandafter\listlen_b\expanded{\loi_normalizeindex{#1}{#2}}{#1}%
}
\def\listlen_b#1#2#3{% #1=err   #2=index normalisé  #3=macroname
	\csname#3len[#2,0]\expandafter\endcsname
	\expanded{\loi_ifempty{#1}{}{\unexpanded{\unexpanded{\loi_error{#1}}}}}%
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%% macro \foreachitem %%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\foreachitem#1\in#2{%
	\edef\foreachitem_a{\noexpand\foreachitem_c\noexpand#1{\expandafter\noexpand\csname\loi_macroname#1cnt\endcsname}{\loi_macroname#2}}%
	\futurelet\loi_nxttok\foreachitem_b
}
\def\foreachitem_b{\loi_ifx{\loi_nxttok[}\foreachitem_a{\foreachitem_a[]}}
\def\foreachitem_c#1#2#3[#4]{% prendre <profondeur max-1>
	\expandafter\foreachitem_d\expanded{\loi_normalizeindex{#3}{#4}}#1{#2}{#3}%
}
\def\foreachitem_d#1#2{\loi_ifempty{#2}{\foreachitem_e{#1}{}}{\foreachitem_e{#1}{#2,}}}% #1=err  #2=index norm
\long\def\foreachitem_e#1#2#3#4#5#6{% #1=err  #2=index norm  #3=macroiter  #4=compteur associé  #5=nom de macrolist  #6=code
	\loi_ifnum{\csname#5len[#20]\endcsname>0 }
		{\loi_ifempty{#1}{}{\loi_error{#1}}%
		\loi_fornum#4=1to\csname#5len[#20]\endcsname\do{\loi_argcsname\let#3{#5[#2#4]}#6}%
		}
		{}%
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%% macro \showitem %%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\showitems{\loi_ifstar{\let\showitems_cmd\detokenize\showitems_a}{\let\showitems_cmd\loi_identity\showitems_a}}
\def\showitems_a#1{\def\showitems_b{\showitems_d#1}\futurelet\loi_nxttok\showitems_c}
\def\showitems_c{\loi_ifx{\loi_nxttok[}\showitems_b{\showitems_b[]}}
\def\showitems_d#1[#2]{\foreachitem\showitems_iter\in#1[#2]{\showitemsmacro{\expandafter\showitems_cmd\expandafter{\showitems_iter}}}}
\unless\ifdefined\fbox
	\newdimen\fboxrule \newdimen\fboxsep \fboxrule=.4pt \fboxsep=3pt % réglages identiques à LaTeX
	\def\fbox#1{% imitation de la macro \fbox de LaTeX, voir pages 271 à 274 de "Apprendre à programmer en TeX"
		\hbox{%
			\vrule width\fboxrule
			\vtop{%
				\vbox{\hrule height\fboxrule \kern\fboxsep \hbox{\kern\fboxsep#1\kern\fboxsep}}%
				\kern\fboxsep \hrule height\fboxrule
			}\vrule width\fboxrule
		}%
	}
\fi
\def\showitemsmacro#1{% encadrement par défaut
	\begingroup\fboxsep=0.25pt \fboxrule=0.5pt \fbox{\strut#1}\endgroup
	\hskip0.25em\relax
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%% macro \itemtomacro %%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\itemtomacro#1[#2]{% #1[#2]=item  non encore lu: #3=macro
	\edef\loi_listname{\loi_macroname#1}%
	\expandafter\itemtomacro_a\expanded{\loi_normalizeindex{\loi_listname}{#2}}\let
}
\def\gitemtomacro#1[#2]{% #1[#2]=item
	\xdef\loi_listname{\loi_macroname#1}%
	\expandafter\itemtomacro_a\expanded{\loi_normalizeindex{\loi_listname}{#2}}{\global\let}%
}
\def\itemtomacro_a#1#2#3#4{%
	\loi_ifempty{#1}{}{\loi_error{#1}}%
	\loi_argcsname#3#4{\loi_listname[#2]}%
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%% réglages par défaut %%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newif\if_removeextremespaces
\newif\if_ignoreemptyitems
\let\ignoreemptyitems\_ignoreemptyitemstrue
\let\reademptyitems\_ignoreemptyitemsfalse
\loi_def_foreachsep{,}
\loi_restorecatcode
\reademptyitems
\setsepchar{,}
\defpair{}
\endinput

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%  historique %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
v1.0    19/8/2016
  - Première version publique
----------------------------------------------------------------------
v1.1    01/09/2016
  - Stockage des séparateurs dans <macrolist>sep
  - bug corrigé dans \loi_restorecatcode
----------------------------------------------------------------------
v1.2    22/10/2016
  - macros \greadlist et \gitemtomacro pour la globalité
----------------------------------------------------------------------
v1.3    18/11/2016
  - bugs corrigés dans la gestion de la globalité
----------------------------------------------------------------------
v1.4    05/10/2017
  - test \loi_ifprimitive ajouté au test \loi_ifcs
  - suppression de \loi_expafternil, création de \loi_expafter,
    modification de \loi_argcsname
  - correction d'un bug : \setsepchar{\par} ne provoque plus d'erreur.
    \loi_ifnum devient \long
----------------------------------------------------------------------
v1.5    06/10/2017
  - correction d'un bug dans \loi_ifcs
----------------------------------------------------------------------
v1.51   24/10/2017
  - correction d'un bug dans \loi_ifcs
----------------------------------------------------------------------
v1.52   13/01/2018
  - le dernier séparateur est <vide>
----------------------------------------------------------------------
v1.53   13/03/2018
  - correction d'un bug dans \readlist_i
----------------------------------------------------------------------
v1.6    01/11/2018
  - possibilité d'appariement de tokens dans les items
----------------------------------------------------------------------
v1.61   03/03/2019
  - la macro \loi_ifcs contient une erreur de conception. Il faut
    tester si le token est un sc && s'il est développable pour
    renvoyer vrai car il existe des sc non développables && qui ne
    sont _pas_ des primitives.
    Macro rebaptisée \loi_ifcsexpandable
----------------------------------------------------------------------
v1.62   18/05/2019
  - utilisation de la nouvelle primitive \expanded au lieu du
    désormais obsolète \romannumeral
  - bug corrigé dans \loi_ifcsexpandable
----------------------------------------------------------------------
v1.63   21/08/2019
  - bug corrigé dans \readlist_h avec les tokens appariés
  - bug corrigé \loi_removefirstspaces est désormais \long

==> listofitemsold.tex <==
% !TeX encoding = ISO-8859-1
% Ce fichier contient le code de l'extension "listofitems"
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                                                    %
\def\loiname                 {listofitems}                           %
\def\loiver                      {1.61}                              %
%                                                                    %
\def\loidate                  {2019/03/03}                           %
%                                                                    %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                                                    %
% Author     : Christian Tellechea, Steven B. Segletes               %
% Status     : Maintained                                            %
% Maintainer : Christian Tellechea                                   %
% Email      : unbonpetit@netc.fr                                    %
%              steven.b.segletes.civ@mail.mil                        %
% Package URL: https://www.ctan.org/pkg/listofitems                  %
% Bug tracker: https://framagit.org/unbonpetit/listofitems/issues    %
% Repository : https://framagit.org/unbonpetit/listofitems/tree/master
% Copyright  : Christian Tellechea 2016-2019                         %
% Licence    : Released under the LaTeX Project Public License v1.3c %
%              or later, see http://www.latex-project.org/lppl.txt   %
% Files      : 1) listofitems.tex                                    %
%              2) listofitems.sty                                    %
%              3) listofitems-fr.tex                                 %
%              4) listofitems-fr.pdf                                 %
%              5) listofitems-en.tex                                 %
%              6) listofitems-en.pdf                                 %
%              7) README                                             %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\ifdefined\ProvidesPackage\else
	\immediate\write -1 {%
	Package: \loidate\space v\loiver\space Grab items in lists using user-specified sep char (CT)}%
\fi

\expandafter\edef\csname loi_restorecatcode\endcsname{\catcode\number`\_=\number\catcode`\_\relax}
\catcode`\_11

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%% gestion des erreurs %%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\ifdefined\PackageError
	\def\loi_error#1{\PackageError\loiname{#1}{Read the manual}}% pour LaTeX
\else
	\def\loi_error#1{\errmessage{Package \loiname\space Error: #1^^J}}% pour TeX
\fi

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%% vérification de la présence de etex %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begingroup
\edef\__tempa{\meaning\eTeXversion}\edef\__tempb{\string\eTeXversion}%
\ifx\__tempa\__tempb
	\endgroup
\else
	\endgroup
	\loi_error{You are not using an eTeX engine, listofitems cannot work.}%
	\loi_restorecatcode\expandafter\endinput
\fi

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%% macros auxiliaires %%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\chardef\loi_stop=0
\def\loi_quark{\loi_quark}
\long\def\loi_identity#1{#1}
\long\def\loi_gobarg#1{}
\long\def\loi_first#1#2{#1}
\long\def\loi_second#1#2{#2}
\long\def\loi_firsttonil#1#2\_nil{#1}
\long\def\loi_antefi#1#2\fi{#2\fi#1}
\long\def\loi_exparg#1#2{\expandafter\loi_exparg_a\expandafter{#2}{#1}}% \loi_exparg{<a>}{<b>} devient <a>{<*b>}
\long\def\loi_exparg_a#1#2{#2{#1}}
\long\def\loi_expafter#1#2{\expandafter\loi_expafter_a\expandafter{#2}{#1}}% \loi_expafter{<a>}{<b>} devient <a><*b>
\long\def\loi_expafter_a#1#2{#2#1}
\def\loi_macroname{\loi_ifinrange\escapechar[[0:255]]{\expandafter\loi_gobarg}{}\string}
\def\loi_argcsname#1#{\loi_argcsname_a{#1}}
\def\loi_argcsname_a#1#2{\loi_expafter{#1}{\csname#2\endcsname}}
\long\def\loi_addtomacro#1#2{\loi_exparg{\def#1}{#1#2}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%% macros de test %%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\long\def\loi_ifnum#1{\ifnum#1\expandafter\loi_first\else\expandafter\loi_second\fi}
\long\def\loi_ifx#1{\ifx#1\expandafter\loi_first\else\expandafter\loi_second\fi}
\long\def\loi_ifempty#1{\loi_exparg\loi_ifx{\expandafter\relax\detokenize{#1}\relax}}
\def\loi_ifstar#1#2{\def\loi_ifstar_a{\loi_ifx{*\loi_nxttok}{\loi_first{#1}}{#2}}\futurelet\loi_nxttok\loi_ifstar_a}
\long\def\loi_ifstuffexpandable#1{\def\loi_tempa{#1}\loi_exparg{\def\loi_tempb}{#1}\expandafter\unless\loi_ifx{\loi_tempa\loi_tempb}}
\long\def\loi_ifcsexpandable#1{% #1 est-il constitué d'une sc _développable_ ?
	\loi_ifempty{#1}
		{\loi_second
		}
		{\loi_ifspacefirst{#1}
			{\loi_second% si espace en 1er, faux
			}
			{%
			\loi_exparg\loi_ifempty{\loi_gobarg#1}% 1 seul token ?
				{\begingroup\escapechar`\_\def\_{#1}\expandafter\endgroup
					\csname loi_\if\expandafter\expandafter\expandafter\loi_firsttonil\expandafter\string\_\_nil\string _first\else second\fi\endcsname
						{\loi_ifstuffexpandable{#1}}
						{\loi_second}%
				}
				{\loi_second% si plusieurs tokens, faux
				}%
			}%
		}%
}
\def\loi_ifinrange#1[[#2:#3]]{\loi_ifnum{\numexpr(#1-#2)*(#1-#3)>0 }\loi_second\loi_first}
\def\loi_ifstring#1\in#2{% si la chaine #1 est contenue dans #2
	\def\loi_ifstring_a##1#1##2\_nil{\loi_ifempty{##2}\loi_second\loi_first}%
	\loi_ifstring_a#2#1\@nil% appel de la macro auxiliaire
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%% macros \loi_foreach %%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcount\loi_cnt_foreach_nest \loi_cnt_foreach_nest=0
\def\end_foreach{\end_foreach}
\def\loi_def_foreachsep#1{%
	\long\def\loi_foreach##1\in##2##3{%
		\global\advance\loi_cnt_foreach_nest1
		\loi_argcsname\def{loop_code_\number\loi_cnt_foreach_nest}{##3}%
		\loi_foreach_a##1##2#1\end_foreach#1%
		\loi_argcsname\let{loop_code_\number\loi_cnt_foreach_nest}\empty
		\global\advance\loi_cnt_foreach_nest-1
	}%
	\long\def\loi_foreach_a##1##2#1{%
		\def##1{##2}%
		\loi_ifx{\end_foreach##1}
			{}
			{\csname loop_code_\number\loi_cnt_foreach_nest\endcsname% exécute le code
			\loi_foreach_a##1%
			}%
	}%
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%% macros gérant l'appariement %%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\long\def\defpair#1{%
	\let\loi_listofpair\empty
	\loi_ifempty{#1}
		{}
		{\defpair_a{}#1\loi_quark\loi_quark}%
}
\long\def\defpair_a#1#2#3{%
	\loi_ifx{\loi_quark#2}
		{\def\loi_sanitizelist##1,\_nil{\def\loi_listofpair{##1}}%
		\loi_sanitizelist#1\_nil
		}
		{\loi_if_validpair#2#3%
			{\long\def\loi_paired_a{#2}\long\def\loi_paired_b{#3}%
			\loi_ifx{\loi_paired_a\loi_paired_b}
				{\loi_error{Paired tokens must not be equal, the pair \detokenize{#2#3} is ignored}%
				\defpair_a{#1}%
				}
				{\defpair_a{#1#2#3,}%
				}%
			}
			{\loi_error{Invalid paired tokens, the pair "\detokenize{#2}" and "\detokenize{#3}" is ignored}%
			\defpair_a{#1}%
			}%
		}%
}
\long\def\loi_if_validpair#1#2{%
	\def\loi_validpair{1}%
	\loi_if_invalid_pairtoken{#1}{\def\loi_validpair{0}}%
	\loi_if_invalid_pairtoken{#2}{\def\loi_validpair{0}}%
	\loi_ifnum{\loi_validpair=1 }
}
\long\def\loi_if_invalid_pairtoken#1{%
	\loi_ifempty{#1}
		{\loi_identity
		}
		{\loi_ifspacefirst{#1}
			{\loi_identity
			}
			{\loi_exparg\loi_ifempty{\loi_gobarg#1}% 1 seul token ?
				{\ifcat\relax\noexpand#1\expandafter\loi_identity\else\expandafter\loi_gobarg\fi}
				{\loi_identity}% si plusieurs tokens, faux
			}%
		}%
}
\long\def\loi_count_occur#1\in#2:#3{% compte le nombre d'occurrences de #1 dans #2 et met le résultat dans la macro #3
	\long\def\loi_count_occur_a##1##2#1##3\_nil{%
		\loi_ifempty{##3}
			{\def#3{##1}}
			{\expandafter\loi_count_occur_a\number\numexpr##1+1\relax##3\_nil}%
	}%
	\loi_count_occur_a0#2#1\_nil
}
\long\def\loi_check_pair#1#2\in#3{% teste l'appariement de #1 et #2 dans #3
	\loi_ifempty{#3}
		{\loi_second
		}
		{\loi_count_occur#1\in#3:\loi_tempa
		\loi_count_occur#2\in#3:\loi_tempb
		\loi_ifnum{\loi_tempa=\loi_tempb\relax}%
		}%
}
\long\def\loi_grabpaired_expr#1#2#3#4#5{% #1=liste de paires  #2=expression  #3=séparateur   #4=résultat    #5=ce qui reste
	\let#4\empty
	\def\loi_remain{#2#3}%
	\loi_foreach\loi_pair\in{#1}{\expandafter\loi_grabpaired_expr_a\loi_pair{#3}#4}%
	\def\loi_remove_lastsep##1#3\_nil{\def#4{##1}}%
	\expandafter\loi_remove_lastsep#4\_nil
	\expandafter\long\expandafter\def\expandafter\loi_grab_remain#4##1\_nil{\loi_ifempty{##1}{\let#5\empty}{\loi_exparg{\def#5}{\loi_gobarg##1}}}%
	\loi_grab_remain#2\_nil
}
\long\def\loi_grabpaired_expr_a#1#2#3#4{% #1#2=paire en cours  #3=séparateur   #4=résultat
	\loi_exparg{\loi_check_pair#1#2\in}#4% si les paires sont appariées dans le résultat
		{}% passer à la paire suivante
		{\long\def\loi_grabpaired_expr_b##1#3##2\_nil{%
			\loi_addtomacro#4{##1#3}% ajouter au résultat ce qui est jusqu'au prochain séparateur
			\def\loi_remain{##2}%
			\loi_exparg{\loi_check_pair#1#2\in}{#4}
				{}
				{\loi_ifempty{##2}
					{\loi_error{"\detokenize{#1}" and "\detokenize{#2}" are not paired}}
					{\loi_grabpaired_expr_b##2\_nil}%
				}%
			}%
		\expandafter\loi_grabpaired_expr_b\loi_remain\_nil
		}%
}
\def\insidepair#1#2#3#4{% #1#2=paire  #3=expr  #4=macro reçevant le resultat
	\loi_if_validpair#1#2%
		{\loi_ifcsexpandable{#3}
			{\loi_exparg{\insidepair#1#2}{#3}#4%
			}
			{\loi_check_pair#1#2\in{#3}% si les paires sont appariées dans le résultat
				{\def\insidepair_a##1#1##2\_nil{\insidepair_b##2\_nil{#1}}%
				\def\insidepair_b##1#2##2\_nil##3{%
					\loi_check_pair#1#2\in{##3##1#2}
						{\loi_exparg{\def#4}{\loi_gobarg##3##1}}%
						{\insidepair_b##2\_nil{##3##1#2}}%
					}%
				\insidepair_a#3\_nil
				}
				{\loi_error{"\detokenize{#1}" and "\detokenize{#2}" are not paired in "#3"}%
				}%
			}%
		}
		{\loi_error{Invalid paired tokens "\detokenize{#1}" and "\detokenize{#2}", empty \string#4 returned}% et bim
		\let#4\empty% voilà, bien fait pour vos gueules
		}%
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%% macro \loi_fornum %%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\loi_fornum#1=#2to#3\do{%
	\edef#1{\number\numexpr#2}\edef\loi_sgncmp{\ifnum#1<\numexpr#3\relax>+\else<-\fi}%
	\expandafter\loi_fornum_a\csname loi_fornum_\string#1\expandafter\endcsname\expandafter{\number\numexpr#3\expandafter}\loi_sgncmp#1%
}
\long\def\loi_fornum_a#1#2#3#4#5#6{\def#1{\unless\ifnum#5#3#2\relax\loi_antefi{#6\edef#5{\number\numexpr#5#41\relax}#1}\fi}#1}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%% macro retirant les espaces extrêmes %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\long\def\loi_ifspacefirst#1{\expandafter\loi_ifspacefirst_a\detokenize{#10} \_nil}
\long\def\loi_ifspacefirst_a#1 #2\_nil{\loi_ifempty{#1}}
\expandafter\def\expandafter\loi_gobspace\space{}
\def\loi_removefirstspaces{\romannumeral\loi_removefirstspaces_a}
\long\def\loi_removefirstspaces_a#1{\loi_ifspacefirst{#1}{\expandafter\loi_removefirstspaces_a\expandafter{\loi_gobspace#1}}{\loi_stop#1}}
\edef\loi_restorezerocatcode{\catcode0=\number\catcode0 \relax}
\catcode0 12
\long\def\loi_removelastspaces#1{\romannumeral\loi_removelastspaces_a#1^^00 ^^00\_nil}
\long\def\loi_removelastspaces_a#1 ^^00{\loi_removelastspaces_b#1^^00}
\long\def\loi_removelastspaces_b#1^^00#2\_nil{\loi_ifspacefirst{#2}{\loi_removelastspaces_a#1^^00 ^^00\_nil}{\loi_stop#1}}
\loi_restorezerocatcode
\long\def\loi_removeextremespaces#1{% #1=texte où les espaces extrêmes sont retirés
	\romannumeral\expandafter\expandafter\expandafter\loi_removelastspaces\expandafter\expandafter\expandafter
	{\expandafter\expandafter\expandafter\loi_stop\loi_removefirstspaces{#1}}%
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%% macro publique \setsepchar %%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\setsepchar{\futurelet\loi_nxttok\setsepchar_a}
\def\setsepchar_a{\loi_ifx{[\loi_nxttok}\setsepchar_b{\setsepchar_b[/]}}
\long\def\setsepchar_b[#1]#2{% #1=sepcar de <liste des sepcar>  #2=<liste des sepcar>
	\loi_ifempty{#1}
		{\loi_error{Empty separator not allowed, separator "/" used}%
		\setsepchar_b[/]{#2}%
		}
		{\def\loi_currentsep{#1}%
		\_removeextremespacesfalse
		\loi_nestcnt1 % réinitaliser niveau initial à 1
		\def\nestdepth{1}%
		\loi_argcsname\let{loi_previndex[\number\loi_nestcnt]}\empty
		\def\loi_listname{loi_listofsep}%
		\let\loi_def\def \let\loi_edef\edef \let\loi_let\let
		\let\loi_listofpair_saved\loi_list_ofpair
		\let\loi_list_ofpair\empty
		\loi_ifempty{#2}
			{\loi_error{Empty list of separators not allowed, "," used}%
			\readlist_e1{,}%
			}
			{\readlist_e1{#2}%
			}%
		\loi_argcsname\let\nestdepth{loi_listofseplen[0]}%
		\loi_argcsname\let\loi_currentsep{loi_listofsep[1]}% 1er car de séparation
		\let\loi_listofpair\loi_listofpair_saved
		}%
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%% macro normalisant l'index %%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\loi_normalizeindex#1#2#3{% #1=macroname  #2=liste d'index  #3=profondeur max --> renvoie {err}{indx norm}
	\loi_ifempty{#2}
		{\loi_stop{}{}}
		{\loi_normalizeindex_a1{}{#3}{#1}#2,\loi_quark,}%
}%
\def\loi_normalizeindex_a#1#2#3#4#5,{% #1=compteur de profondeur #2=index précédents  #3=profondeur max #4=macroname  #5=index courant
	\loi_ifx{\loi_quark#5}
		{\loi_normalizeindex_c#2\loi_quark% supprimer la dernière virgule
		}
		{\loi_ifnum{#1>#3 }
			{\loi_invalidindex{Too deeply nested index, index [.] retained}{#2}% si profondeur trop grande
			}
			{\loi_ifinrange\ifnum\numexpr#5<0 -1*\fi(#5)[[1:\csname #4len[#20]\endcsname]]% si abs(#5) hors de [1,len]
				{\loi_exparg\loi_normalizeindex_b{\number\numexpr#5\ifnum\numexpr#5<0 +\csname #4len[#20]\endcsname+1\fi}{#1}{#2}{#3}{#4}}
				{\loi_invalidindex{#5 is an invalid index, index [.] retained}{#2}}%
			}%
		}%
}
\def\loi_normalizeindex_b#1#2#3{\loi_exparg\loi_normalizeindex_a{\number\numexpr#2+1}{#3#1,}}% #1=index à rajouter  #2=compteur de profondeur #3=index précédents
\def\loi_normalizeindex_c#1,\loi_quark{\loi_stop{}{#1}}
\def\loi_invalidindex#1#2{\loi_ifempty{#2}{\loi_invalidindex_a{#1},}\loi_invalidindex_a{#1}{#2}}
\def\loi_invalidindex_a#1#2{\loi_invalidindex_b#1\loi_quark#2\loi_quark}
\def\loi_invalidindex_b#1[.]#2\loi_quark#3,\loi_quark#4\loi_quark,{\loi_stop{#1[#3]#2}{#3}}% #4= index ignorés

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%% macro publique \readlist %%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcount\loi_nestcnt
\def\greadlist{\let\loi_def\gdef\let\loi_edef\xdef\def\loi_let{\global\let}\readlist_a}%
\def\readlist{\let\loi_def\def\let\loi_edef\edef\let\loi_let\let\readlist_a}
\def\readlist_a{%
	\loi_nestcnt1 % niveau initial = 1
	\loi_argcsname\let{loi_previndex[\number\loi_nestcnt]}\empty
	\loi_ifstar{\_removeextremespacestrue\readlist_b}{\_removeextremespacesfalse\readlist_b}%
}
\long\def\readlist_b#1#2{% #1=macro stockant les éléments  #2=liste des éléments
	\loi_ifcsexpandable{#2}
		{\loi_exparg{\readlist_b#1}{#2}%
		}
		{\loi_edef\loi_listname{\loi_macroname#1}%
		\loi_argcsname\loi_let{\loi_listname nest}\nestdepth
		\loi_argcsname\loi_def{\loi_listname[]}{#2}% la liste entière
		\loi_argcsname\loi_def{\loi_listname sep[]}{}% séparateur vide
		\loi_ifempty{#2}
			{\loi_def#1[##1]{}%
			\loi_argcsname\loi_def{\loi_listname len}{0}\loi_argcsname\loi_def{\loi_listname len[0]}{0}%
			\loi_error{Empty list ignored, nothing to do}%
			}
			{\loi_edef#1[##1]{\unexpanded{\romannumeral\expandafter\loi_checkindex\romannumeral\loi_normalizeindex}{\loi_listname}{##1}{\csname\loi_listname nest\endcsname}{\loi_listname}}%
			\loi_argcsname\loi_edef{\loi_listname sep}[##1]{\unexpanded{\romannumeral\expandafter\loi_checkindex\romannumeral\loi_normalizeindex}{\loi_listname}{##1}{\csname\loi_listname nest\endcsname}{\loi_listname sep}}%
			\readlist_c{#2}%
			\loi_argcsname\loi_argcsname\loi_let{\loi_listname len}{\loi_listname len[0]}% longueur du niveau 0
			}%
		}%
}
\def\loi_checkindex#1#2#3{%
	\expandafter\expandafter\expandafter\loi_stop\csname#3[#2]\expandafter\endcsname
	\romannumeral\loi_ifempty{#1}{\loi_stop}{\loi_stop\loi_error{#1}}%
}
\def\readlist_c{%
	\loi_argcsname\loi_let\loi_currentsep{loi_listofsep[\number\loi_nestcnt]}%
	\expandafter\readlist_d\loi_currentsep||\_nil
}
\long\def\readlist_d#1||#2\_nil#3{\readlist_e1{#3#1}}% #1=<sep courant simple>  #3=liste -> rajoute un élément vide pour le test \ifempty ci dessous
\long\def\readlist_e#1#2{% #1=compteur d'index  #2=liste d'éléments à examiner terminée par <sep courant simple> >>RIEN laissé après
	\loi_ifempty{#2}
		{\loi_argcsname\loi_edef{\loi_listname len[\csname loi_previndex[\number\loi_nestcnt]\endcsname0]}{\number\numexpr#1-1\relax}%
		\loi_argcsname\loi_let{\loi_listname sep[\csname loi_previndex[\number\loi_nestcnt]\endcsname\number\numexpr#1-1\relax]}\empty% le dernier <sep> est <vide> ##NEW v1.52
		\advance\loi_nestcnt-1
		\loi_argcsname\loi_let\loi_currentsep{loi_listofsep[\number\loi_nestcnt]}%
		}
		{\loi_expafter{\readlist_f{#2}{}}\loi_currentsep||\loi_quark||#2\_nil{#1}% aller isoler le 1er item
		}%
}
\long\def\readlist_f#1#2#3||{% #1=liste restante   #2=<dernier sep utilisé>  #3=<sep courant>
	\loi_ifx{\loi_quark#3}% on a épuisé tous les <séparateurs> ? RESTE à lire <expr+sep1>\_nil{<compteur>}
		{\loi_ifempty{#2}% si #2 vide, aucun <sep utilisé> n'a été trouvé, il reste à lire "<liste complète>\_nil"
			{\long\def\readlist_g##1\_nil##2{\loi_exparg{\readlist_h{##2}{}}{\loi_gobarg##1}{#2}}% ##2=compteur d'index
			}
			{\loi_ifx{\loi_listofpair\empty}% paires définies ?
				{\long\def\readlist_g##1#2##2\_nil##3{\loi_exparg{\readlist_h{##3}{##2}}{\loi_gobarg##1}{#2}}%
				}
				{\long\def\readlist_g##1\_nil##2{%
					\loi_exparg{\loi_exparg\loi_grabpaired_expr\loi_listofpair}{\loi_gobarg##1}{#2}\loi_grabpaired_result\loi_grabpaired_remain
					\loi_exparg{\loi_exparg{\readlist_h{##2}}{\loi_grabpaired_remain}}{\loi_grabpaired_result}{#2}}%
				}%
			}%
		\readlist_g\relax% le \relax meuble l'argument délimité
		}
		{\long\def\readlist_g##1#3##2\_nil{%
			\loi_ifempty{##2}% si <liste restante> ne contient pas le <sep courant>
				{\readlist_f{#1}{#2}% recommencer avec le même <sep utile>
				}%
				{\loi_ifx{\loi_listofpair\empty}% si pas de paires définies
					{\loi_exparg\readlist_f{\loi_gobarg##1#3}{#3}% raccourcir <liste restante> et <sep courant>:=<sep utile>% ##BUGFIX v1.53
					}%
					{\loi_exparg\loi_grabpaired_expr\loi_listofpair{#1}{#3}\loi_grabpaired_result\loi_grabpaired_remain
					\loi_exparg\readlist_f{\loi_grabpaired_result#3}{#3}%
					}%
				}%
			}%
		\readlist_g\relax#1#3\_nil% ##BUGFIX v1.53
		}%
}
\long\def\readlist_h#1#2#3{% #1=compteur d'index  #2=liste restante  #3=élément courant
	\loi_ifnum{0\loi_exparg\loi_ifspacefirst{\loi_currentsep}{}1\if_removeextremespaces1\fi=11 }% s'il faur retirer les espaces extrêmes
		{\loi_exparg{\loi_exparg{\readlist_i{#1}{#2}}}{\loi_removeextremespaces{#3}}}% redéfinir l'élément courant
		{\readlist_i{#1}{#2}{#3}}%
}
\long\def\readlist_i#1#2#3#4{% #1=compteur d'index  #2=liste restante  #3=élément courant   #4=sep utilisé
	\loi_ifnum{0\if_ignoreemptyitems1\fi\loi_ifempty{#3}1{}=11 }
		{\readlist_e{#1}{#2}% si l'on n'ignore pas les éléments vides
		}%
		{\loi_argcsname\loi_def{\loi_listname[\csname loi_previndex[\number\loi_nestcnt]\endcsname#1]}{#3}% assignation de l'item ctuel à la macro
		\loi_argcsname\loi_def{\loi_listname sep[\csname loi_previndex[\number\loi_nestcnt]\endcsname#1]}{#4}% assignation du <sep> actuel à la macro \<macrolist>sep
		\loi_ifnum{\loi_nestcnt<\nestdepth\relax}% si imbrication max non atteinte
			{\advance\loi_nestcnt1
			\loi_argcsname\edef{loi_previndex[\number\loi_nestcnt]}{\csname loi_previndex[\number\numexpr\loi_nestcnt-1]\endcsname#1,}%
			\readlist_c{#3}% recommencer avec l'élément courant
			}
			{}%
		\loi_exparg\readlist_e{\number\numexpr#1+1}{#2}% puis chercher l'élément suivant dans la liste restante
		}%
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%% macro \listlen %%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\listlen#1[#2]{%
	\romannumeral\loi_ifempty{#2}
		{\expandafter\expandafter\expandafter\loi_stop\csname\loi_macroname#1len[0]\endcsname}
		{\loi_exparg\listlen_a{\romannumeral-`\.\loi_macroname#1}{#2}}%
}
\def\listlen_a#1#2{% #1=macro name   #2=index non normalisé    prendre <profondeur max-1>
	\loi_exparg{\expandafter\listlen_b\romannumeral\loi_normalizeindex{#1}{#2}}{\number\numexpr\csname#1nest\endcsname-1}{#1}%
}
\def\listlen_b#1#2#3{% #1=err   #2=index normalisé  #3=macroname
	\expandafter\expandafter\expandafter\loi_stop\csname#3len[#2,0]\expandafter\endcsname
	\romannumeral\loi_ifempty{#1}{\loi_stop}{\loi_stop\loi_error{#1}}%
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%% macro \foreachitem %%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\foreachitem#1\in#2{%
	\edef\foreachitem_a{\noexpand\foreachitem_c\noexpand#1{\expandafter\noexpand\csname\loi_macroname#1cnt\endcsname}{\loi_macroname#2}}%
	\futurelet\loi_nxttok\foreachitem_b
}
\def\foreachitem_b{\loi_ifx{\loi_nxttok[}\foreachitem_a{\foreachitem_a[]}}
\def\foreachitem_c#1#2#3[#4]{% prendre <profondeur max-1>
	\loi_exparg{\expandafter\foreachitem_d\romannumeral\loi_normalizeindex{#3}{#4}}{\number\numexpr\csname#3nest\endcsname-1}#1{#2}{#3}%
}
\def\foreachitem_d#1#2{\loi_ifempty{#2}{\foreachitem_e{#1}{}}{\foreachitem_e{#1}{#2,}}}% #1=err  #2=index norm
\long\def\foreachitem_e#1#2#3#4#5#6{% #1=err  #2=index norm  #3=macroiter  #4=compteur associé  #5=nom de macrolist  #6=code
	\loi_ifnum{\csname#5len[#20]\endcsname>0 }
		{\loi_ifempty{#1}{}{\loi_error{#1}}%
		\loi_fornum#4=1to\csname#5len[#20]\endcsname\do{\loi_argcsname\let#3{#5[#2#4]}#6}%
		}
		{}%
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%% macro \showitem %%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\showitems{\loi_ifstar{\let\showitems_cmd\detokenize\showitems_a}{\let\showitems_cmd\loi_identity\showitems_a}}
\def\showitems_a#1{\def\showitems_b{\showitems_d#1}\futurelet\loi_nxttok\showitems_c}
\def\showitems_c{\loi_ifx{\loi_nxttok[}\showitems_b{\showitems_b[]}}
\def\showitems_d#1[#2]{\foreachitem\showitems_ater\in#1[#2]{\showitemsmacro{\expandafter\showitems_cmd\expandafter{\showitems_ater}}}}
\unless\ifdefined\fbox
	\newdimen\fboxrule \newdimen\fboxsep \fboxrule=.4pt \fboxsep=3pt % réglages identiques à LaTeX
	\def\fbox#1{% imitation de la macro \fbox de LaTeX, voir pages 271 à 274 de "Apprendre à programmer en TeX"
		\hbox{%
			\vrule width\fboxrule
			\vtop{%
				\vbox{\hrule height\fboxrule \kern\fboxsep \hbox{\kern\fboxsep#1\kern\fboxsep}}%
				\kern\fboxsep \hrule height\fboxrule
			}\vrule width\fboxrule
		}%
	}
\fi
\def\showitemsmacro#1{% encadrement par défaut
	\begingroup\fboxsep=0.25pt \fboxrule=0.5pt \fbox{\strut#1}\endgroup
	\hskip0.25em\relax
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%% macro \itemtomacro %%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\itemtomacro#1[#2]{% #1[#2]=item  non encore lu: #3=macro
	\edef\loi_listname{\loi_macroname#1}%
	\loi_exparg{\expandafter\itemtomacro_a\romannumeral\expandafter\loi_normalizeindex\expandafter{\loi_listname}{#2}}{\csname\loi_listname nest\endcsname}\let
}
\def\gitemtomacro#1[#2]{% #1[#2]=item
	\xdef\loi_listname{\loi_macroname#1}%
	\loi_exparg{\expandafter\itemtomacro_a\romannumeral\expandafter\loi_normalizeindex\expandafter{\loi_listname}{#2}}{\csname\loi_listname nest\endcsname}{\global\let}%
}
\def\itemtomacro_a#1#2#3#4{%
	\loi_ifempty{#1}{}{\loi_error{#1}}%
	\loi_argcsname#3#4{\loi_listname[#2]}%
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%% réglages par défaut %%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newif\if_removeextremespaces
\newif\if_ignoreemptyitems
\let\ignoreemptyitems\_ignoreemptyitemstrue
\let\reademptyitems\_ignoreemptyitemsfalse
\setsepchar{,}
\defpair{}
\loi_def_foreachsep{,}
\reademptyitems

\loi_restorecatcode
\endinput

######################################################################
############################  Historique #############################
######################################################################

v1.0  19/8/2016
  - Première version publique

v1.1  01/09/2016
  - Stockage des séparateurs dans <macrolist>sep
  - bug corrigé dans \loi_restorecatcode

v1.2  22/10/2016
  - macros \greadlist et \gitemtomacro pour la globalité

v1.3  18/11/2016
  - bugs corrigés dans la gestion de la globalité

v1.4  05/10/2017
  - test \loi_ifprimitive ajouté au test \loi_ifcs
  - suppression de \loi_expafternil, création de \loi_expafter,
    modification de \loi_argcsname
  - correction d'un bug : \setsepchar{\par} ne provoque plus
    d'erreur. \loi_ifnum devient \long

v1.5  06/10/2017
  - correction d'un bug dans \loi_ifcs

v1.51 24/10/2017
  - correction d'un bug dans \loi_ifcs

v1.52 13/01/2018
  - le dernier séparateur est <vide>

v1.53 13/03/2018
  - correction d'un bug dans \readlist_g

v1.6 01/11/2018
  - possibilité d'appariement de tokens dans les items
  
v1.61 03/03/2019
    - la macro \loi_ifcs contient une erreur de conception.
      Il faut tester si le token est un sc && s'il est
      développable pour renvoyer vrai car il existe des sc
      non développables && qui ne sont _pas_ des primitives.
      Macro rebaptisée \loi_ifcsexpandable
